Quantifying & Modeling Multimodal Interactions: An Information Decomposition Framework

The recent explosion of interest in multimodal applications has resulted in a wide selection of datasets and methods for representing and integrating information from different modalities. Despite these empirical advances, there remain fundamental research questions: How can we quantify the interactions that are necessary to solve a multimodal task? Subsequently, what are the most suitable multimodal models to capture these interactions? To answer these questions, we propose an information-theoretic approach to quantify the degree of redundancy, uniqueness, and synergy relating input modalities with an output task. We term these three measures as the PID statistics of a multimodal distribution (or PID for short), and introduce two new estimators for these PID statistics that scale to high-dimensional distributions. To validate PID estimation, we conduct extensive experiments on both synthetic datasets where the PID is known and on large-scale multimodal benchmarks where PID estimations are compared with human annotations. Finally, we demonstrate their usefulness in (1) quantifying interactions within multimodal datasets, (2) quantifying interactions captured by multimodal models, (3) principled approaches for model selection, and (4) three real-world case studies engaging with domain experts in pathology, mood prediction, and robotic perception where our framework helps to recommend strong multimodal models for each application.

==> figures/overview.tex <==
\begin{figure}[tbp]
\centering
\vspace{-6mm}
\includegraphics[width=0.9\linewidth]{figures/overview_fig.pdf}
\vspace{-2mm}
\caption{The \name\ framework formalizes the nature of feature interactions for a task. Through our proposed scalable estimators for \textit{redundancy}, \textit{uniqueness}, and \textit{synergy}, we demonstrate its usefulness towards quantifying multimodal datasets, model predictions, and model selection.}
\label{fig:overview}
\vspace{-4mm}
\end{figure}

==> figures/robust.tex <==
\begin{figure}[tbp]
\centering
\vspace{-0mm}
\includegraphics[width=0.8\linewidth]{figures/unimodal_robust.pdf}
\vspace{-6mm}
\caption{We find high correlation ($0.62$) between the performance drop when $X_i$ is missing and the model's $U_i$ value: high $U_i$ coincides with large performance drops, but low $U_i$ can also lead to performance drops. The latter can be further explained by the presence of large $R$ and $S$ values despite low $U_i$ which also causes performance drops.}
\label{fig:robust}
\vspace{-4mm}
\end{figure}

==> tables/compare.tex <==
\begin{table*}[t]
\centering
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{3.0pt}
\vspace{-0mm}
\caption{Comparison between \esta\ and \estb\ on selected real-world datasets.}
\centering
\footnotesize
\vspace{-2mm}

\begin{tabular}{l|cccc|cccc}
\hline \hline
Task & \multicolumn{4}{c|}{\textsc{AV-MNIST}} & \multicolumn{4}{c}{\textsc{Push i,c}} \\
\hline
Measure & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn \\
\hline
\esta & $0.10$ & $0.97$ & $0.03$ & $0.08$ & $0.24$ & $0.03$ & $0.06$ & $0.04$ \\
\estb & $0.40$ & $1.04$ & $0.04$ & $0.16$ & $0.75$ & $1.79$ & $0.03$ & $0.08$ \\
\hline \hline
\end{tabular}
\label{tab:comp_batch}
\end{table*}

==> tables/gmm.tex <==
\begin{table*}[t]
\centering
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{3.0pt}
\vspace{-2mm}
\caption{Results on estimating \name\ across different GMM}
\centering
\footnotesize
\vspace{-2mm}

\begin{tabular}{l|cccc|cccc|cccc|cccc|cccc}
\hline \hline
Category & \multicolumn{4}{c|}{\textsc{General}} & \multicolumn{16}{c}{\textsc{Redundancy}} \\
\hline
Model & \multicolumn{4}{c|}{\textsc{EF}} & \multicolumn{4}{c|}{\textsc{Additive}} & \multicolumn{4}{c|}{\textsc{Agree}} & \multicolumn{4}{c|}{\textsc{Align}} & \multicolumn{4}{c}{\textsc{SSL}} \\
\hline
Measure & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn \\
\hline
ur-funny {a,t} & 0.02 & 0 & 0.02 & 0.06 & 0.02 & 0 & 0.02 & 0.15 & 0.02 & 0 & 0.02 & 0.05 & 0.02 & 0 & 0.02 & 0.06 & &  &  & \\
ur-funny {v,t} & 0.05 & 0.01 & 0 & 0.17 & 0.11 & 0.08 & 0 & 0.17 & 0.02 & 0.04 & 0 & 0.24 & 0.02 & 0 & 0.02 & 0.15 & &  &  & \\
ur-funny {v,a} & 0.01 & 0.27 & 0 & 0.19 & 0.03 & 0 & 0.02 & 0.15 &  0.02 & 0 & 0.02 & 0.15 & 0.12 & 0.05 & 0.01 & 0.19 & &  &  & \\
mosei t,a & 0.03 & 0 & 0.05 & 0.02 & 0.02 & 0 & 0.03 & 0.02 & 0.02 & 0 & 0.03 & 0.02 & 0.02 & 0 & 0 & 0.02 & & &  &\\
mosei t,v & 0 & 0 & 0 & 0 & 0.02 & 0 & 0.02 & 0.02 & 0.02 & 0 & 0.03 & 0.02 & 0.03 & 0 & 0 & 0.03 & & &  &\\
mosei a,v & 0 & 0 & 0 & 0 & 0.08 & 0.01 & 0 & 0.02 & 0.07 & 0 & 0 & 0.02 & 0.13 & 0 & 0.02 & 0.02 & & &  &\\
mimic & 0.01 & 0.27 & 0 & 0 & 0.01 & 0.27 & 0 & 0 & 0.01 & 0.27 & 0 & 0 & 0.01 & 0.28 & 0 & 0 & &  &  &   \\
avmnist \\
push \\
enrico & 0.71 & 0.34 & 0.44 & 0.38 & 0.69 & 0.28 & 0.39 & 0.35
 & & & &  & 0.40 & 0.30 & 0.52 & 0.75 & &  &  &  \\
vqa \\
clevr \\
Average & \\
\hline \hline
\end{tabular}

\vspace{4mm}

\begin{tabular}{l|cccc|cccc|cccc|cccc|cccc}
\hline \hline
Category & \multicolumn{4}{c|}{\textsc{General}} & \multicolumn{16}{c}{\textsc{Redundancy}} \\
\hline
Model & \multicolumn{4}{c|}{\textsc{EF}} & \multicolumn{4}{c|}{\textsc{Additive}} & \multicolumn{4}{c|}{\textsc{Agree}} & \multicolumn{4}{c|}{\textsc{Align}} & \multicolumn{4}{c}{\textsc{SSL}} \\
\hline
Measure & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn \\
\hline
$(z_c)$ & 0.47 & 0.01 & 0.01 & 0.04 & 0.56 & 0.01 & 0.01 & 0.03 & 0.56 & 0.01 & 0 & 0.03 & 0.57 & 0.01 & 0.01 & 0.03 \\
$(z_1)$ & 0 & 0.41 & 0 & 0.04 & 0.01 & 0.02 & 0 & 0.06 & 0.07 & 0.44 & 0 & 0.02 & 0.02 & 0.13 & 0 & 0.08 \\
$(z_2)$ & 0.01 & 0 & 0.47 & 0.04 & 0.01 & 0 & 0.58 & 0.01 & 0.01 & 0 & 0.59 & 0.01 & 0.01 & 0 & 0.59 & 0.01 \\
$(z_1,z_2)$ & 0.15 & 0.02 & 0 & 0.29 & 0.1 & 0 & 0.19 & 0.25 & 0.1 & 0 & 0.18 & 0.26 & 0.1 & 0 & 0.17 & 0.27 \\
$(z_1^*,z_2^*,z_c^*)$ & 0.22 & 0 & 0.07 & 0.15 & 0.29 & 0 & 0.16 & 0.11 & 0.28 & 0 & 0.15 & 0.12 & 0.3 & 0 & 0.15 & 0.13 \\
$(z_1,z_2^*,z_c^*)$ & 0.16 & 0.15 & 0 & 0.15 & 0.2 & 0 & 0.06 & 0.09 & 0.13 & 0 & 0.11 & 0.09 & 0.18 & 0 & 0.06 & 0.09 \\
$(z_1,z_2,z_c^*)$ & 0.16 & 0.05 & 0 & 0.25 & 0.15 & 0 & 0.25 & 0.13 & 0.15 & 0 & 0.22 & 0.13 & 0.16 & 0 & 0.25 & 0.11 \\
$(z_1^*,z_2^*,z_c)$ & 0.25 & 0.03 & 0 & 0.14 & 0.44 & 0 & 0.04 & 0.1 & 0.41 & 0 & 0.08 & 0.07 & 0.42 & 0 & 0.07 & 0.1 \\
$(z_2^*,z_c^*)$ & 0.19 & 0 & 0.12 & 0.06 & 0.2 & 0 & 0.27 & 0.03 & 0.22 & 0 & 0.32 & 0.02 & 0.18 & 0 & 0.32 & 0.03 \\
$(z_2^*,z_c)$ & 0.26 & 0 & 0.12 & 0.05 & 0.37 & 0 & 0.18 & 0.04 & 0.34 & 0 & 0.17 & 0.04 & 0.35 & 0 & 0.19 & 0.04 \\
\hline \hline
\end{tabular}

\vspace{4mm}

\begin{tabular}{l|cccc|cccc|cccc|cccc|cccc|cccc}
\hline \hline
Category & \multicolumn{16}{c|}{\textsc{Synergy}} & \multicolumn{8}{c}{\textsc{Unique}} \\
\hline
Model & \multicolumn{4}{c|}{\textsc{Elem}} & \multicolumn{4}{c|}{\textsc{Outer}} & \multicolumn{4}{c|}{\textsc{MI}} & \multicolumn{4}{c|}{\textsc{MulT}} & \multicolumn{4}{c|}{\textsc{Lower}} & \multicolumn{4}{c}{\textsc{Rec}} \\
\hline
Measure & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn \\
\hline
ur-funny t,a & 0.01 & 0 & 0.03 & 0.05 & 0.01 & 0 & 0.02 & 0.05 & 0.01 & 0 & 0.03 & 0.04 & & & & & 0.02 & 0 & 0.01 & 0.14 & 0.01 & 0 & 0.02 & 0.04 \\
ur-funny t,v & 0.02 & 0.01 & 0 & 0.16 & 0.03 & 0.01 & 0 & 0.14 & 0.04 & 0.02 & 0 & 0.14 & & & & & 0.04 & 0 & 0.01 & 0.15 & 0.03 & 0.01 & 0 & 0.17 \\
ur-funny a,v & 0.03 & 0.13 & 0 & 0.16 & 0.02 & 0.15 & 0 & 0.15 & 0.02 & 0.23 & 0 & 0.15 & & & & & 0.02 & 0.15 & 0 & 0.19 & 0.05 & 0.08 & 0 & 0.20 \\
mosei t,a & 0.02 & 0 & 0.03 & 0.02 & 0.02 & 0 & 0.03 & 0.02 & 0.02 & 0 & 0.02 & 0.02 & & & & & 0.02 & 0 & 0.04 & 0.02 \\
mosei t,v & 0.01 & 0 & 0.04 & 0.03 & 0.01 & 0 & 0.04 & 0.03 & 0.03 & 0 & 0.03 & 0.03 & & & & & 0.02 & 0 & 0.04 & 0.03 & &  &\\
mosei a,v & 0.03 & 0.02 & 0 & 0.02 & 0.02 & 0.01 & 0 & 0.01 & 0.03 & 0.01 & 0 & 0.02 & & & & & 0.02 & 0.01 & 0 & 0.01 \\
mimic & 0.04 & 0.24 & 0 & 0.01 & 0 & 0.28 & 0 & 0.01 & 0.02 & 0.26 & 0 & 0.01 & & & & & 0.01 & 0.28 & 0 & 0.01 & 0.03 & 0 & 0.03 & 0.11 \\
avmnist \\
push \\
enrico & 0.3 & 0.43 & 0.29 & 0.73 & 0.38 & 0.48 & 0.32 & 0.69 & 0.56 & 0.28 & 0.41 & 0.34 & & & & & 0.38 & 0.52 & 0.29 & 0.69 & \\
vqa \\
clevr \\
Average & \\
\hline \hline
\end{tabular}

\vspace{4mm}

\begin{tabular}{l|cccc|cccc|cccc|cccc|cccc|cccc}
\hline \hline
Category & \multicolumn{16}{c|}{\textsc{Synergy}} & \multicolumn{8}{c}{\textsc{Unique}} \\
\hline
Model & \multicolumn{4}{c|}{\textsc{Elem}} & \multicolumn{4}{c|}{\textsc{Outer}} & \multicolumn{4}{c|}{\textsc{MI}} & \multicolumn{4}{c|}{\textsc{MulT}} & \multicolumn{4}{c|}{\textsc{Lower}} & \multicolumn{4}{c}{\textsc{Rec}} \\
\hline
Measure & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn & \red & \uone & \utwo & \syn \\
\hline
$(z_c)$ & 0.22 & 0 & 0 & 0.06 & 0.30 & 0 & 0.01 & 0.05 & 0.22 & 0.02 & 0 & 0.06 & 0.4 & 0.02 & 0 & 0.06 & 0.34 & 0 & 0.01 & 0.06 & 0.56 & 0 & 0.03 & 0.04 \\
$(z_1)$ & 0 & 0.15 & 0 & 0.05 & 0 & 0.26 & 0 & 0.05 & 0.01 & 0.14 & 0 & 0.05 & 0 & 0.48 & 0 & 0.02 & 0.01 & 0.26 & 0 & 0.05 & 0.01 & 0.55 & 0 & 0.02 \\
$(z_2)$ & 0.01 & 0 & 0.19 & 0.05 & 0 & 0 & 0.25 & 0.06 & 0.01 & 0 & 0.14 & 0.05 & 0.02 & 0 & 0.41 & 0.06 & 0 & 0 & 0.28 & 0.05 & 0.01 & 0 & 0.5 & 0.02 \\
$(z_1,z_2)$ & 0.08 & 0.01 & 0 & 0.16 & 0.10 & 0.01 & 0 & 0.19 & 0.04 & 0.01 & 0 & 0.1 & 0.16 & 0.05 & 0 & 0.29 & 0.07 & 0.02 & 0 & 0.16 & 0.15 & 0.06 & 0 & 0.35 \\
$(z_1^*,z_2^*,z_c^*)$ & 0.04 & 0 & 0 & 0.07 & 0.07 & 0.01 & 0 & 0.06 & 0.01 & 0 & 0.01 & 0.04 & 0.21 & 0.11 & 0 & 0.2 & 0.06 & 0.01 & 0 & 0.05 & 0.2 & 0.04 & 0 & 0.25 \\
$(z_1,z_2^*,z_c^*)$ & 0.05 & 0.05 & 0 & 0.07 & 0.07 & 0.03 & 0 & 0.06 & 0.03 & 0.02 & 0 & 0.06 & 0.1 & 0.29 & 0 & 0.11 & 0.05 & 0.06 & 0 & 0.06 & 0.11 & 0.24 & 0 & 0.2 \\
$(z_1,z_2,z_c^*)$ & 0.08 & 0.02 & 0 & 0.11 & 0.06 & 0 & 0.01 & 0.1 & 0.05 & 0.01 & 0 & 0.08 & 0.18 & 0.02 & 0 & 0.3 & 0.09 & 0 & 0 & 0.11 & 0.17 & 0.08 & 0 & 0.31 \\
$(z_1^*,z_2^*,z_c)$ & 0.11 & 0 & 0 & 0.09 & 0.14 & 0 & 0 & 0.06 & 0.12 & 0.01 & 0.01 & 0.06 & 0.33 & 0 & 0.03 & 0.14 & 0.15 & 0 & 0 & 0.06 & 0.35 & 0.04 & 0 & 0.19 \\
$(z_2^*,z_c^*)$ & 0.04 & 0 & 0.03 & 0.05 & 0.08 & 0.01 & 0 & 0.05 & 0.02 & 0 & 0.01 & 0.06 & 0.13 & 0 & 0.4 & 0.04 & 0.07 & 0 & 0.01 & 0.06 & 0.15 & 0 & 0.36 & 0.03 \\
$(z_2^*,z_c)$ & 0.15 & 0 & 0.03 & 0.06 & 0.18 & 0 & 0.02 & 0.06 & 0.13 & 0 & 0.01 & 0.06 & 0.36 & 0 & 0.18 & 0.04 & 0.25 & 0 & 0 & 0.06 & 0.37 & 0 & 0.18 & 0.03 \\
\hline \hline
\end{tabular}


\vspace{-4mm}
\label{tab:models}
\end{table*}
